Towards Efficient Synthesis of Quantum Graph States by Fusing Graph Motifs

Photonic graph states with advanced topologies can enable measurement-based quantum computing, distributed quantum sensing, and quantum interconnects. However, the efficient generation of photonic graph states is limited by the probabilistic nature of photonic entangling operations and the exponential dependence of generation rate on resource cost. In this work, we study photonic graph state synthesis as a cost-aware decomposition problem, exploiting local Clifford (LC) equivalence to identify more synthesis-friendly representations of the target graph state before decomposition. Specifically, we propose Cost-aware Fusion-based Decomposition (CFD), a three-stage heuristic framework that decomposes a target graph state into ring, star, and linear motifs, and assembles them via Type-I fusion operations to minimize fusion overhead and physical-qubit consumption. We further show that selecting the LC-equivalent graph state with the minimum number of edges provides a highly effective proxy for near-optimal synthesis: in many cases it matches the best generation rate observed within the LC equivalence class under CFD, and in most remaining cases it remains close to it. Numerical evaluations on graph state orbit data and 2D and 3D lattice graph states demonstrate that CFD achieves up to 84.6\% reduction in resource overhead compared to baseline constructions, and yields improvements in photonic generation rate spanning multiple orders of magnitude. These results suggest that combining structure-aware motif decomposition with LC equivalence is a practical and scalable strategy for photonic graph state synthesis.

==> Dima.tex <==
\section{Dima}\label{Dima}

The experimental approach for the generation of graph states with complex topologies involves the first generation of base graph states, namely graph states with chain (one-dimensional cluster state) and star (GHZ) topologies, and then fusing the base graph states to achieve the desired topology.

The generation of one-dimensional cluster states can be performed by realizing the Lindner-Rudolph circuit shown in Fig. XXX. We denote the photon qubits in the cluster states in the basis of their circular polarization states, $|R\rangle$ and $|L\rangle$ and a solid state single photon emitter (atom, ion, or quantum dot) trapped in the basis of its two ground-state energy levels, $|\uparrow\rangle$> and $|\downarrow\rangle$>. According to the circuit, the generation of photonic cluster states requires two operations (gates) applied on the photons and the spin: $\pi/2$-gates on the spin and controlled not (CNOT) gates that flip the state of a photon only for one of the spin states (e.g., the photon state $|R\rangle$ stays $|R\rangle$ for spin $|\uparrow\rangle$ but transfers to $|L\rangle$ for spin $|\downarrow\rangle$). The realization of $\pi/2$-gate on the spin is possible by applying an optical or microwave pulse of coherent control or by applying a small external magnetic field and waiting for a quarter spin precession. Meanwhile, to realize CNOT gates on the photons based on the spin state requires a repeated pulsed excitation and leveraging of optical selection rules, i.e., the emitter will decay to different spin states based on the polarization of the photon. . The emitted photons are the qubits in the cluster state. This polarization dependence means that the repeated optical excitations not only produce the photons, but they also entangle the photon with the spin, which is equivalent to the realization of a CNOT gate.
The generation of GHZ states is similar to the generation of one-dimensional cluster states but does not require spin precession). 
Despite the successful generation of one-dimensional cluster states using such gates, the number of entangled photons in the cluster was limited to 10, and the rates of generating photons were limited to 500 MHz [2,17], which is insufficient for fusing the cluster states into complex graph states [7, 9].

Figure X: Generation and fusing of base graph states. 

To experimentally generate graph states with complex topologies requires the realization of three types of operations on one-dimensional cluster states and GHZ states  as exemplified in Figure 4. The first type of operation is local Clifford operations on a qubit, which can be realized by a rotation of the photon polarization utilizing quarter and half waveplates or an electrical polarization controller. The second type of operations is projective measurements that can have three different effects on photons from a cluster state (illustrated in Fig. 4a): a “Z” projective measurement on a photon (i.e., its circular polarization component) cuts its entanglement links to adjacent photons, an “X” measurement (horizontal polarization component) combines adjacent photons to a single encoded redundant photon, and a “Y” measurement on a photon (diagonal polarization component) links it to the adjacent qubits. Following the approach proposed by Browne and Rudolph [9], the third type of operations applied on photons from two separate clusters are “fusion gates”. Specifically, we will realize a “type-II fusion gate” by interfering the photons on a polarizing beamsplitter and detecting photons at the two output ports of the beamsplitter. As illustrated in Fig. XXXX, the implementation of a type II fusion gate has two possible outcomes with a 50\% probability. The first outcome is when a single photon is detected in each of the beamsplitter’s output ports, indicating the success of the fusion attempt. The second outcome is when zero or two photons are detected at each of the beamsplitter’s output ports. While this outcome fails to fuse the one-dimensional cluster states, Browne and Rudolph showed that it will prepare a redundant photon in the second one-dimensional cluster state . Thus, even if the first attempt to fuse the cluster states fails, a second type II fusion gate can be implemented on the redundant photon. As described in detail in section 4.5.1, m repeated fusion attempts on redundant photons will increase the probability of succeeding in the fusion operation as p=1-12m, thereby boosting the probability of generating the desired graph state in a single shot. Nevertheless, considering our high single photon generation rates and realistic photon losses, it might be faster (on average) to regenerate all photons rather than reattempting fusion.


 Such an entanglement can be achieved by either performing local operations and measurements on individual photons in a simple graph state such as a one-dimensional cluster state or a start topology Greenberger–Horne –Zeilinger (GHZ) state, or by “fusing” separate simple graph states into a more complex topology

Coupling quantum dots to nanophotonic cavities has resulted in the emission of single photons with sub-100 ps lifetimes. 

If our experimental setup has an overall photon collection efficiency of $\eta$, then the total rate to generate a graph state with $N$ photons will be given by $R=\frac{R_1\times\eta^N}{N}$ (and without $/N$ for streams). 

Here, by boosting collection efficiency up to = 0.4 provided by the cavity and improved optical setup, and by choosing a single photon generation rate of $R_1=6$ GHz, we will be able to generate $N=6$ entangled photons at a rate of R~ 25 MHz, N=7 entangled photons at a rate of R~ 10 MHz, and N=10 entangled photons at a rate of R~ 630 kHz. 

For protocols that involve fusion operations, we will sacrifice two photons (from one-dimensional cluster states or GHZ states) per fusion attempt. Considering a 50\% success of fusion operations, the successful generation of a graph states with $N$ photons using one fusion operation will require two attempts (on average) to generate the whole state while post selecting the successful states, resulting in generation rates of $R\approx \frac{1}{2(N+2)}\times R_1\times \eta^{N+2}$ (without $/N$ for a stream). 

Hence, a collection efficiency of $\eta=0.4$ and a single photon generation rate of R1= 6 GHz will allow us to generate graph states with N=6 entangled photons with one fusion gate at an (average) rate of R~ 2 MHz. 

This reduction of rates due to the probabilistic nature of the fusion operations highlights the importance of  developing algorithms for achieving graph states based on more local operations and less fusion gates. 

The generation of a  graph state with a complex topology and N=10 photons may be achievable at an (average) rate of R~ 630 kHz if no fusion gates are needed, R~ 50 kHz if a single fusion gate is needed, and R~ 4 kHz if two fusion gates are needed. 

Alternatively, if we wish to increase the probability of generating the correct state in a single shot (rather than trying to generate the same state twice and post-selecting on the successful generation), then we need to perform more fusion operations on redundant photons within a single production of the one-dimensional cluster state. Thus, attempting the same fusion operation $m$ times (while sacrificing $2\times m$ photons) will result in a generation rate of RpR1N+2m, with p=1-12m is the probability to generate the correct states in a single shot (50\% with one fusion attempt, 75\% with two fusion attempts etc.). As a result, enhancing the average rate of generating desired graph states in a single shot (rather than by post selection) will require the improvement of the photon collection efficiency of the setup.

